Tracing Content Requirements in Financial Documents using Multi-granularity Text Analysis

The completeness (in terms of content) of financial documents is a fundamental requirement for investment funds. To ensure completeness, financial regulators have to spend significant time carefully checking every financial document based on relevant content requirements, which prescribe the information types to be included in financial documents (e.g., the description of shares' issue conditions and procedures). However, existing techniques provide limited support to help regulators automatically identify the text chunks related to financial information types, due to the complexity of financial documents. In this paper, we propose FITI to trace content requirements in financial documents with multi-granularity text analysis. Given a new financial document, FITI first selects a set of candidate sentences for efficient information type identification. Then, to rank candidate sentences, FITI uses a combination of rule-based and data-centric approaches, by leveraging information retrieval (IR) and machine learning (ML) techniques that analyze the words, sentences, and contexts related to an information type. Finally, a heuristic-based selector, which considers both the sentence ranking and domain-specific phrases, determines a list of sentences corresponding to each information type. We evaluated FITI by assessing its effectiveness in tracing financial content requirements in 100 real-world financial documents. Experimental results show that FITI is able to provide accurate identification with average precision, recall, and F1-score values of 0.824, 0.646, and 0.716, respectively. The overall accuracy of FITI significantly outperforms the best baseline (based on a transformer language model) by 0.266 in terms of F1-score. Furthermore, FITI can help regulators detect about 80% of missing information types in financial documents

==> pics/analysis-flow.tex <==

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]
\tikzstyle{rect} = [rectangle, minimum width=1.5cm,  text centered, text width=1.5cm, draw=black, fill=white!30]
\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, text centered, text width=4cm, draw=white, fill= white!30]
\tikzstyle{text_model} = [rectangle, minimum width=0.8cm, text centered, text width=0.8cm, draw=white, fill= white!30]

\tikzstyle{list_box} = [rect,align=left ,minimum width=2.39cm,text width=3.19cm, minimum height= 0.5cm]

\resizebox{1\textwidth}{!}{
	\begin{tikzpicture} [node distance=0.3mm, >=latex]
	
	\node (labeled1) [rect, text
	width=2.0cm]{$s^L_{1r_t}, \dots, s^L_{ir_t}$};
	\node (labeled_text1) [rect, draw=none, below = of labeled1, text width=3.3cm] {Related sentences $S^L_{r_t}$};
	
	\node (vec_group) [rect, right = of labeled1, minimum width=1cm, text
	width=1.8cm, xshift=0.7cm]{group\\vector};
				
	\node (similar1) [round_rect, right = of vec_group, minimum width=1cm, text
	width=1.7cm, xshift=0.7cm]{cosine similarity};
	
	\node (vec_context_1) [rect, right = of similar1, minimum width=1cm, text
	width=1.5cm, xshift=0.7cm]{context vector};
	\node (candidate_text) [rect, draw=none, below = of vec_context_1, text width=2.5cm] {Candidate sentence $s_i$};
	
	\draw [arrow,->] (labeled1) -- (vec_group);
	\draw [arrow, ->] (vec_group) -- (similar1);
	\draw [arrow, ->] (vec_context_1) -- (similar1);
	
	\node (sim_sg) [text_node, below = of similar1, minimum width=1.5cm, text width=1.5cm, yshift=-1.0cm]{\color{blue}{$s.\mathit{group}$}};
	\draw [arrow,->] (similar1) -- (sim_sg);
	\node (example1) [rect, draw=none, below = of sim_sg, text width=3.3cm, xshift=-1.5cm, yshift=-0.2cm] {(A) Group similarity};
	
%------------------------
	\node (labeled2) [rect, right = of vec_context_1, text
	width=2.0cm, xshift=1cm]{$s^L_{1r_t}, \dots, s^L_{ir_t}$};
	\node (labeled_text2) [rect, draw=none, below = of labeled2, text width=3.3cm] {Related sentences $S^L_{r_t}$};
	
	\node (vec_si) [rect, right = of labeled2, minimum width=1cm, text
	width=3.3cm, xshift=0.7cm]{context vector of $s^L_{ir_t}$};
	\node (vec_sn) [text_node, draw=none, above= of vec_si, text width=3cm]{$\cdots\cdots$};
	\node (vec_s1) [rect, above = of vec_sn, minimum width=1cm, text
	width=3.3cm]{context vector of $s^L_{1r_t}$};
	
	\node (similar2) [round_rect, right = of vec_si, minimum width=1cm, text
	width=1.7cm, xshift=0.7cm]{cosine similarity};
	
	\node (vec_context_2) [rect, right = of similar2, minimum width=1cm, text
	width=1.5cm, xshift=0.7cm]{context vector};
	\node (candidate_text) [rect, draw=none, below = of vec_context_2, text width=2.5cm] {Candidate sentence $s_i$};
	
	\draw [arrow,->] (labeled2.east) -- (vec_s1.west);
	\draw [arrow,->] (labeled2) -- (vec_si);
	\draw [arrow,->] (vec_si) -- (similar2);
	\draw [arrow,->] (vec_s1.east) -- (similar2.west);
	\draw [arrow,->] (vec_context_2) -- (similar2);
	
	\node (sim_ss) [text_node, below = of similar2, minimum width=1.5cm, text
	width=1.5cm, yshift=-1.0cm]{\color{blue}{$s.\mathit{avg\_s}$, $s.\mathit{max\_s}$}};
	\draw [arrow,->] (similar2) -- (sim_ss);
	\node (example2) [rect, draw=none, right = of example1, text width=3.5cm, xshift=7.5cm] {(B) Sentence similarity};
%------------------------
\node (labeled3) [rect, below = of labeled1, text
width=2.0cm, yshift=-4cm]{$s^L_{1r_t}, \dots, s^L_{ir_t}$};
\node (labeled_text3) [rect, draw=none, below = of labeled3, text width=3.3cm] {Related sentences $S^L_{r_t}$};

\node (vec_imp) [rect, right = of labeled3, minimum width=1cm, text
width=1.8cm, xshift=0.7cm]{$\mathit{imp}(w)$ of words};

\node (similar3) [round_rect, right = of vec_imp, minimum width=1cm, text
width=1.7cm, xshift=0.7cm]{importance similarity};

\node (vec_context_3) [rect, right = of similar3, minimum width=1cm, text
width=1.5cm, xshift=0.7cm]{words in $s_i$};
\node (candidate_text) [rect, draw=none, below = of vec_context_3, text width=2.5cm] {Candidate sentence $s_i$};

\draw [arrow,->] (labeled3) -- (vec_imp);
\draw [arrow,->] (vec_imp) -- (similar3);
\draw [arrow,->] (vec_context_3) -- (similar3);

\node (sim_imp) [text_node, below = of similar3, minimum width=1.5cm, text
width=1.5cm, yshift=-1.0cm]{\color{blue}{$s.\mathit{word}$}};
\draw [arrow,->] (similar3) -- (sim_imp);

\node (example3) [rect, draw=none, below = of example1, text width=5cm, yshift=-5.2cm] {(C) Word importance similarity};

%------------------------
\node (labeled4) [rect, below = of labeled2, text
width=2.1cm, yshift=-4cm]{$s^L_{1r_t}, \dots, s^L_{ir_t}$};
\node (labeled_text4) [rect, draw=none, below = of labeled4, text width=3.3cm] {Related sentences $S^L_{r_t}$};

\node (vec_posi) [rect, right = of labeled4, minimum width=1cm, text
width=3.3cm, xshift=0.7cm]{feature vector of $s^L_{ir_t}$};
\node (vec_posn) [text_node, draw=none, above= of vec_posi, text width=3cm]{$\cdots\cdots$};
\node (vec_pos1) [rect, above = of vec_posn, minimum width=1cm, text
width=3.3cm]{feature vector of $s^L_{1r_t}$};

\node (similar4) [round_rect, right = of vec_posi, minimum width=1cm, text
width=1.7cm, xshift=0.7cm]{Random forest};

\node (vec_context_4) [rect, right = of similar4, minimum width=1cm, text
width=1.5cm, xshift=0.7cm]{feature vector};
\node (candidate_text) [rect, draw=none, below = of vec_context_4, text width=2.5cm] {Candidate sentence $s_i$};

\draw [arrow,->] (labeled4) -- (vec_posi);
\draw [arrow,->] (vec_posi) -- (similar4);
\draw [arrow,->] (labeled4.east) -- (vec_pos1.west);
\draw [arrow,->] (vec_pos1.east) -- (similar4.west);

\node (labeled4_neg) [rect, below = of labeled4, text
width=2.1cm, yshift=-1.5cm]{$s^L_{1u_t}, \dots, s^L_{iu_t}$};
\node (labeled_text4_neg) [rect, draw=none, below = of labeled4_neg, text width=3.7cm] {Unrelated sentences $S^L_{u_t}$};

\node (vec_negi) [rect, right = of labeled4_neg, minimum width=1cm, text
width=3.3cm, xshift=0.7cm]{feature vector of $s^L_{iu_t}$};
\node (vec_negn) [text_node, draw=none, above= of vec_negi, text width=3cm]{$\cdots\cdots$};
\node (vec_neg1) [rect, above = of vec_negn, minimum width=1cm, text
width=3.3cm]{feature vector of $s^L_{1u_t}$};

\draw [arrow,->] (labeled4_neg) -- (vec_negi);
\draw [arrow,->] (vec_negi.east) -- (similar4.west);
\draw [arrow,->] (labeled4_neg.east) -- (vec_neg1.west);
\draw [arrow,->] (vec_neg1.east) -- (similar4.west);
\draw [arrow,->] (vec_context_4) -- (similar4);

\node (sim_pos) [text_node, below = of similar4, minimum width=1.5cm, text
width=1.5cm, yshift=-1.0cm]{\color{blue}{$s.\mathit{ml}$}};
\draw [arrow,->] (similar4) -- (sim_pos);

\node (example4) [rect, draw=none, below = of example2, text width=5cm, yshift=-5.2cm] {(D) Feature-based probability};

	\end{tikzpicture}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/candidates-flow.tex <==

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]
\tikzstyle{rect} = [rectangle, minimum width=1.5cm,  text centered, text width=1.5cm, draw=black, fill=white!30]
\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, text centered, text width=4cm, draw=white, fill= white!30]
\tikzstyle{text_model} = [rectangle, minimum width=0.8cm, text centered, text width=0.8cm, draw=white, fill= white!30]

\tikzstyle{list_box} = [rect,align=left ,minimum width=2.39cm,text width=3.19cm, minimum height= 0.5cm]

\resizebox{1\textwidth}{!}{
	\begin{tikzpicture} [node distance=0.3mm, >=latex]
	
	\node (doc) [rect, draw=none, text width=3cm]{ \includegraphics[width=\textwidth]{pics/snippet.png}};
	\node (doc_text) [rect, draw=none, below = of doc, text width=4cm] {Unlabeled document $d$};
	
	\node (s1) [text_node, right= = of doc, minimum width=0.3cm, text width=0.3cm, xshift=2cm, yshift=1cm]{$s_1$:};
	\node (s1_text) [text_node, right= = of s1, text
	width=7.3cm, xshift=2.5cm, yshift=1cm, align=left]{\dots\emph{subfund close new subscript application}\dots};
	
	\node (s2) [text_node, right= = of doc, minimum width=0.3cm, text width=0.3cm, xshift=2cm, yshift=0cm]{$s_2$:};
	\node (s2_text) [text_node, right= = of s2, text
	width=7.3cm, xshift=2.5cm, yshift=0cm, align=left]{\dots\emph{applicable maximum sale charge levy}\dots};
	
	\node (s3) [text_node, right= = of doc, minimum width=0.3cm, text width=0.3cm, xshift=2cm, yshift=-1cm]{$s_3$:};
	\node (s3_text) [text_node, right= = of s3, text
	width=7.3cm, xshift=2.5cm, yshift=-1cm, align=left]{\dots\emph{subscript application submit written form}\dots};
			
	\node (s0) [text_node, draw=none, above= of s1_text, text
	width=7.3cm]{$\cdots\cdots$};
	
	\node (sn) [text_node, draw=none, below= of s3_text, text
	width=7.3cm]{$\cdots\cdots$};
	
	
	\draw [arrow,->] (doc) -- (s1);
	\draw [arrow,->] (doc) -- (s2);
	\draw [arrow,->] (doc) -- (s3);
	
	\node (s1_v) [rect, right= of s1_text, text
	width=5.3cm, xshift=0.7cm]{\dots 4.2, 2.6, 0.0, 8.0, \dots, 3.0, 0.0, 5.0 \dots};
	
	\node (s2_v) [rect, right= of s2_text, text
	width=5.3cm, xshift=0.7cm]{\dots 6.3, 2.6, 1.0, 8.0, \dots, 3.0, 2.2, 7.5 \dots};
	
	\node (s3_v) [rect, right= of s3_text, text
	width=5.3cm, xshift=0.7cm]{\dots 2.1, 0.0, 1.0, 8.0, \dots, 0.0, 2.2, 2.5 \dots};
	
	\node (s_v_text) [rect, draw=none, below = of s3_v, text width=5.3cm] {The context vector of each sentence using TF-IDF measurement};
		
	\node (sg_v) [rect, above= of s1_v, text
	width=5.3cm, yshift=1.49cm]{\dots 8.4, 2.6, 3.0, 0.0, \dots, 1.5, 8.8, 7.5 \dots};
	
	\node (voc1) [text_node, above= of sg_v,minimum width=0.3cm, text width=0.3cm, xshift=-2.4cm, yshift=0.3cm, rotate around={45:(0,0)}, ]{$\cdots$};
	\node (voc2) [text_node, right= of voc1,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{application};
	\node (voc3) [text_node, right= of voc2,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{close};
	\node (voc4) [text_node, right= of voc3,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{form};
	\node (voc5) [text_node, right= of voc4,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{levy};
	\node (voc6) [text_node, right= of voc5,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{$\cdots$};
	\node (voc7) [text_node, right= of voc6,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{subfund};
	\node (voc8) [text_node, right= of voc7,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{submit};
	\node (voc9) [text_node, right= of voc8,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{subscript};
	\node (voc10) [text_node, right= of voc9,minimum width=0.3cm, text width=0.3cm, rotate around={45:(0.55,0)}]{$\cdots$};
	
	\node (voc_text) [text_node, above = of sg_v, text width=1.3cm, yshift=1.5cm] {\textbf{Vocabulary}};
		

	\node (point_s1_text) [text_node, minimum width=0.0cm, text width=0.0cm, right = of s1_text, xshift=-0.6cm] {};
	\node (point_s2_text) [text_node, minimum width=0.0cm, text width=0.0cm, right = of s2_text, xshift=-0.6cm] {};
	\node (point_s3_text) [text_node, minimum width=0.0cm, text width=0.0cm, right = of s3_text, xshift=-0.6cm] {};
	\node (point_s1_v) [text_node, minimum width=0.0cm, text width=0.0cm, left = of s1_v, xshift=0.0cm] {};
	\node (point_s2_v) [text_node, minimum width=0.0cm, text width=0.0cm, left = of s2_v, xshift=0.0cm] {};
	\node (point_s3_v) [text_node, minimum width=0.0cm, text width=0.0cm, left = of s3_v, xshift=0.0cm] {};
	\node (point_s0_text) [text_node, minimum width=0.0cm, text width=0.0cm, above = of point_s1_text, yshift=0.2cm] {};
	\node (point_sn_text) [text_node, minimum width=0.0cm, text width=0.0cm, below = of point_s3_text, yshift=-0.2cm] {};
	\draw [arrow,->] (point_s1_text) -- (point_s1_v);
	\draw [arrow,->] (point_s2_text) -- (point_s2_v);
	\draw [arrow,->] (point_s3_text) -- (point_s3_v);
	\draw [arrow,->, dashed] (point_s1_text) -- (point_s2_v);
	\draw [arrow,->, dashed] (point_s2_text) -- (point_s1_v);
	\draw [arrow,->, dashed] (point_s2_text) -- (point_s3_v);
	\draw [arrow,->, dashed] (point_s3_text) -- (point_s2_v);
	\draw [arrow,->, dashed] (point_s0_text) -- (point_s1_v);
	\draw [arrow,->, dashed] (point_sn_text) -- (point_s3_v);
	
	\node (labeled) [rect, above= = of doc, text
	width=2.5cm, yshift=3.12cm]{$s^L_{1r_t}, \dots, s^L_{ir_t}$};
	\node (labeled_text) [rect, draw=none, below = of labeled, text width=5.3cm] {Related sentences $S^L_{r_t}$};
	\node (point_s_labeled) [text_node, minimum width=0.0cm, text width=0.0cm, left = of sg_v, xshift=0.0cm] {};
	\draw [arrow,->] (labeled) -- node [anchor=south] {Group vector}(point_s_labeled);
	
	\draw [arrow,<->] (sg_v) -- (s1_v);
	\node (point_cosine) [text_node, minimum width=0.0cm, text width=0.0cm, above = of s1_v, yshift=0.6cm, xshift=-0.14cm] {};
	
	\node (s_set) [rect, right= of s1_v, text
	width=2.0cm, yshift=1.22cm, xshift=0.5cm]{$s_1, s_2, s_{10}, \dots$};
	\node (s_set_text) [rect, draw=none, below = of s_set, text width=2.3cm] {Candidate sentences};
	\draw [arrow,->] (point_cosine) -- node [anchor=south] {Cosine similarity}(s_set);

	\node (big_box)[draw=black, fit={(s0)(s1)(s1_text)(s2)(s2_text)(s3)(s3_text)(sn)},minimum width=1.4cm,text width=7.3cm, minimum height=2.5cm, xshift=-0.2cm]{};
	
	\node (s_process) [rect, draw=none, below = of big_box, text width=5.3cm] {Preprocessed sentences};
	
	\end{tikzpicture}
      }



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/figure-rq-component.tex <==

\subfloat[Precision of \approach and its variants]{
	\label{fig:rq-component-p}{
		\begin{tikzpicture}
		[scale=0.46]
		\begin{axis} [ybar = .05cm,
		bar width = 6pt,
		xmin = 0,
		xmax = 6,
		ymax = 1,
		enlarge x limits = {value = .25},
		xticklabels={T1, T2, T3, T4, T5},
		xtick={1,...,5},
		ylabel={Precision},
		ylabel near ticks,
                axis y discontinuity=parallel,
		legend pos=north west,
		]

		\addplot table [x=ID, y=FITI-IR-P, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{IR}$};
		\addplot table [x=ID, y=FITI-ML-P, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{ML}$};
		\addplot table [x=ID, y=FITI-P, col sep=comma] {data/rq-component.csv};
		\addlegendentry{\approach};

		\end{axis}
		\end{tikzpicture}
	}
}
\hfill
\subfloat[Recall of \approach and its variants]{
	\label{fig:rq-component-r}{
		\begin{tikzpicture}
		[scale=0.46]
		\begin{axis} [ybar = .05cm,
		bar width = 6pt,
		xmin = 0,
		xmax = 6,
		ymax = 1,
		enlarge x limits = {value = .25},
		xticklabels={T1, T2, T3, T4, T5},
		xtick={1,...,5},
		ylabel={Recall},
		ylabel near ticks,
                axis y discontinuity=parallel,
		legend pos=north west,
		]

		\addplot table [x=ID, y=FITI-IR-R, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{IR}$};
		\addplot table [x=ID, y=FITI-ML-R, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{ML}$};
		\addplot table [x=ID, y=FITI-R, col sep=comma] {data/rq-component.csv};
		\addlegendentry{\approach};

		\end{axis}
		\end{tikzpicture}
	}
}
\hfill
\subfloat[F$_1$-score of \approach and its variants]{
	\label{fig:rq-component-f}{
		\begin{tikzpicture}
		[scale=0.46]
		\begin{axis} [ybar = .05cm,
		bar width = 6pt,
		xmin = 0,
		xmax = 6,
		ymax = 1,
		enlarge x limits = {value = .25},
		xticklabels={T1, T2, T3, T4, T5},
		xtick={1,...,5},
		ylabel={F$_1$-score},
		ylabel near ticks,
                axis y discontinuity=parallel,
		legend pos=north west,
		]

		\addplot table [x=ID, y=FITI-IR-F, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{IR}$};
		\addplot table [x=ID, y=FITI-ML-F, col sep=comma] {data/rq-component.csv};\addlegendentry{$\text{\approach}_\mathit{ML}$};
		\addplot table [x=ID, y=FITI-F, col sep=comma] {data/rq-component.csv};
		\addlegendentry{\approach};

		\end{axis}
		\end{tikzpicture}
	}
      }


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/figure-rq-train-size.tex <==

\subfloat[Precision of \approach]{
	\label{fig:rq-train-size-p}
	\begin{tikzpicture}[scale=0.46]
		\begin{axis}[
			xlabel={Number of training documents},
			ylabel={Precision},
			ylabel near ticks,
			xmin=0, xmax=100,
			legend style={
				at={(0.5,-0.2)},
				anchor=north,
				legend columns=-1
			},
			ymajorgrids=true,
                        axis y discontinuity=parallel,
			grid style=dashed,
			cycle list={
				solid, every mark/.append style={solid, fill=red}, mark=*\\%
				dotted, every mark/.append style={solid, fill=green}, mark=square*\\%
				densely dotted, every mark/.append style={solid, fill=blue}, mark=otimes*\\%
				loosely dotted, every mark/.append style={solid, fill=cyan}, mark=triangle*\\%
				dashed, every mark/.append style={solid, fill=yellow},mark=diamond*\\%
				loosely dashed, every mark/.append style={solid, fill=olive},mark=*\\%
				densely dashed, every mark/.append style={solid, fill=orange},mark=square*\\%
				dashdotted, every mark/.append style={solid, fill=gray},mark=otimes*\\%
				dasdotdotted, every mark/.append style={solid, fill=brown},mark=star\\%
				densely dashdotted,every mark/.append style={solid, fill=teal},mark=diamond*\\%
			},
			]

			\addplot table [x=ID, y=T1, col sep=comma] {data/rq-train-size-p.csv};\addlegendentry{T1};
			\addplot table [x=ID, y=T2, col sep=comma] {data/rq-train-size-p.csv};\addlegendentry{T2};
			\addplot table [x=ID, y=T3, col sep=comma] {data/rq-train-size-p.csv};
			\addlegendentry{T3};
			\addplot table [x=ID, y=T4, col sep=comma] {data/rq-train-size-p.csv};
			\addlegendentry{T4};
			\addplot table [x=ID, y=T5, col sep=comma] {data/rq-train-size-p.csv};
			\addlegendentry{T5};

		\end{axis}
	\end{tikzpicture}
}
\hfill
\subfloat[Recall of \approach]{
	\label{fig:rq-train-size-r}
	\begin{tikzpicture}[scale=0.46]
		\begin{axis}[
		%title={The effect of number of filled fields},
		xlabel={Number of training documents},
		ylabel={Recall},
		ylabel near ticks,
		xmin=0, xmax=100,
		legend style={
			at={(0.5,-0.2)},
			anchor=north,
			legend columns=-1
		},
		ymajorgrids=true,
                axis y discontinuity=parallel,
		grid style=dashed,
		cycle list={
			solid, every mark/.append style={solid, fill=red}, mark=*\\%
			dotted, every mark/.append style={solid, fill=green}, mark=square*\\%
			densely dotted, every mark/.append style={solid, fill=blue}, mark=otimes*\\%
			loosely dotted, every mark/.append style={solid, fill=cyan}, mark=triangle*\\%
			dashed, every mark/.append style={solid, fill=yellow},mark=diamond*\\%
		},
		]

		\addplot table [x=ID, y=T1, col sep=comma] {data/rq-train-size-r.csv};\addlegendentry{T1};
		\addplot table [x=ID, y=T2, col sep=comma] {data/rq-train-size-r.csv};\addlegendentry{T2};
		\addplot table [x=ID, y=T3, col sep=comma] {data/rq-train-size-r.csv};
		\addlegendentry{T3};
		\addplot table [x=ID, y=T4, col sep=comma] {data/rq-train-size-r.csv};
		\addlegendentry{T4};
		\addplot table [x=ID, y=T5, col sep=comma] {data/rq-train-size-r.csv};
		\addlegendentry{T5};

		\end{axis}
	\end{tikzpicture}
}
\hfill
\subfloat[F$_1$-score of \approach]{
	\label{fig:rq-train-size-f}
	\begin{tikzpicture}[scale=0.46]
		\begin{axis}[
		xlabel={Number of training documents},
		ylabel={F$_1$-score},
		ylabel near ticks,
		xmin=0, xmax=100,
		legend style={
			at={(0.5,-0.2)},
			anchor=north,
			legend columns=-1
		},
		ymajorgrids=true,
                axis y discontinuity=parallel,
		grid style=dashed,
		cycle list={
			solid, every mark/.append style={solid, fill=red}, mark=*\\%
			dotted, every mark/.append style={solid, fill=green}, mark=square*\\%
			densely dotted, every mark/.append style={solid, fill=blue}, mark=otimes*\\%
			loosely dotted, every mark/.append style={solid, fill=cyan}, mark=triangle*\\%
			dashed, every mark/.append style={solid, fill=yellow},mark=diamond*\\%
		},
		]

		\addplot table [x=ID, y=T1, col sep=comma] {data/rq-train-size-f.csv};\addlegendentry{T1};
		\addplot table [x=ID, y=T2, col sep=comma] {data/rq-train-size-f.csv};\addlegendentry{T2};
		\addplot table [x=ID, y=T3, col sep=comma] {data/rq-train-size-f.csv};
		\addlegendentry{T3};
		\addplot table [x=ID, y=T4, col sep=comma] {data/rq-train-size-f.csv};
		\addlegendentry{T4};
		\addplot table [x=ID, y=T5, col sep=comma] {data/rq-train-size-f.csv};
		\addlegendentry{T5};

		\end{axis}
	\end{tikzpicture}
}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/snippet.tex <==

\tikzstyle{round_rect} = [rectangle, rounded corners, minimum width=1.5cm, minimum height=0.5 cm,text centered, draw=black, fill=white!30]
\tikzstyle{rect} = [rectangle, minimum width=1.5cm, minimum height=0.8cm, text centered, text width=1.5cm, draw=black, fill=white!30]
\tikzstyle{text_node} = [rectangle, minimum width=0.5cm, minimum height=0.35cm, text centered, text width=4cm, draw=white, fill= white!30]

\resizebox{0.48\textwidth}{!}{
	\begin{tikzpicture} [node distance=5mm, >=latex]

		% A page of financial document
		\node (page)[inner sep=0pt]
		{\includegraphics[width=.13\textwidth]{pics/page.png}};
		\node (locate) [draw=blue, minimum width=1.0cm, minimum height=1.1cm, line width=0.2mm, right = of page, xshift=-1.5cm, yshift=-0.4cm] {};
		\node (ptext)[text_node, minimum width=0.2cm, below= of page, yshift=0.5cm] {A page of financial document};

		\draw[fill=blue!10, ] (1.0,0.2) -- (1.0,-1) -- (1.4,-1.7) -- (1.4,3.6)
		-- cycle;

		% A snippet with information types
		\node (snippet)[inner sep=0pt, right=of page, yshift= 1cm]
		{\includegraphics[width=.5\textwidth]{pics/snippet.png}};
		\node (method) [text_node, minimum width=0.3cm, above= of snippet, yshift=-0.2cm, xshift=-2cm] {Calculation method for issue price};
		\node (issue) [text_node, minimum width=0.3cm, above= of snippet, yshift=-0.2cm, xshift=2cm] {Issue conditions and procedures};
		\node (point1)[draw=white, below = of method, yshift=0.2cm]{};
		\node (point2)[draw=white, below = of issue, yshift=-3.6cm]{};
		\draw [arrow, ->, thick] (method)--(point1);
		\draw [arrow, ->, thick] (issue)--(point2);

	\end{tikzpicture}
}


==> pics/table-annotation.tex <==
	\pgfplotstabletypeset[
		every head row/.style={
		before row=\toprule,
		after row=\midrule,
	},
	every nth row={2}{before row=\midrule},
	every last row/.style={
	after row=\bottomrule},
	columns/Phase/.style ={column name={\textbf{Phase}}, column type={p{.1\textwidth}}}, 
	columns/Type/.style ={column name={\textbf{Issue Type}}, column type={p{.15\textwidth}}}, 	
	columns/Meaning/.style ={column name={\textbf{Meaning}}, column type={p{.2\textwidth}}}, 
	columns/Solution/.style ={column name={\textbf{Solution}}, column type={p{.4\textwidth}}}, 
	col sep=ampersand,
	string type,
	]{data/annotation-info.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-dataset.tex <==
\pgfplotstabletypeset[
	every head row/.style={
		before row=\toprule,
		after row=\midrule,
	},
%	every nth row={4}{before row=\midrule},
	every last row/.style={
		after row=\bottomrule},
		columns/Key/.style ={column name={Item}}, 
		columns/Value/.style ={column name={Value}
	}, 
	col sep=comma,
	string type,
]{data/dataset-info.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-features.tex <==
	\pgfplotstabletypeset[
	every head row/.style={
		before row=\toprule,
		after row=\midrule,
	},
	every nth row={1}{before row=\midrule},
	every last row/.style={
		after row=\bottomrule},
	columns/ID/.style ={column name={\textbf{ID}}}, 
	columns/Details/.style ={column name={\textbf{Name (N), Type (T), Description (D), and Intuition (I)}}, column type={p{.9\textwidth}}}, 	
	col sep=ampersand,
	string type,
	]{data/feature-info.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-rq-accuracy.tex <==
\pgfplotstabletypeset[
	every head row/.style={
		before row={%
			\toprule
			\multirow{2.8}{*}{ID}&\multicolumn{4}{c}{Precision}&\multicolumn{4}{c}{Recall}&\multicolumn{4}{c}{F$_1$-score}\\
			\cmidrule(l){2-5}
			\cmidrule(lr){6-9}
			\cmidrule(r){10-13}
		},
		after row=\midrule,
	},
	every last row/.style={
		after row=\bottomrule
	},
	every nth row={5}{before row=\midrule},
	columns/ID/.style ={column name=}, 
	columns/P-KW/.style ={column name=KW}, 
	columns/P-BERT/.style ={column name=BERT}, 
	columns/P-BERTKW/.style ={column name=BERT$_\mathit{KW}$}, 
	columns/P-FITI/.style={column name=\approach}, 
	columns/R-KW/.style ={column name=KW},
	columns/R-BERT/.style ={column name=BERT}, 
	columns/R-BERTKW/.style ={column name=BERT$_\mathit{KW}$}, 
	columns/R-FITI/.style={column name=\approach},	 
	columns/F-KW/.style ={column name=KW},
	columns/F-BERT/.style ={column name=BERT}, 
	columns/F-BERTKW/.style ={column name=BERT$_\mathit{KW}$}, 
	columns/F-FITI/.style ={column name=\approach},
	col sep=comma,
	string type,
]{data/rq-accuracy.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-rq-inspection.tex <==
\pgfplotstabletypeset[
	every head row/.style={
		before row={%
			\toprule
%			ID&Precision&Recall&F$_1$-score\\
		},
		after row=\midrule,
	},
	every last row/.style={
		after row=\bottomrule
	},
	every nth row={5}{before row=\midrule},
	columns/ID/.style ={column name=ID}, 
	columns/P/.style ={column name=Precision}, 
	columns/R/.style ={column name=Recall},
	columns/F/.style ={column name=F$_1$-score},
	col sep=comma,
	string type,
]{data/rq-inspection.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-rq-selection.tex <==
\pgfplotstabletypeset[
	every head row/.style={
		before row={%
			\toprule
			\multirow{2.5}{*}{ID}&\multicolumn{4}{c}{Precision}&\multicolumn{4}{c}{Recall}&\multicolumn{4}{c}{F$_1$-score}\\
			\cmidrule(l){2-5}
			\cmidrule(lr){6-9}
			\cmidrule(r){10-13}
		},
		after row=\midrule,
	},
	every last row/.style={
		after row=\bottomrule
	},
	every nth row={5}{before row=\midrule},
	columns/ID/.style ={column name=}, 
	columns/P-SC/.style ={column name=\approach{$_{\mathit{score}}$}}, 
	columns/P-TN/.style={column name=\approach{$_{\mathit{topN}}$}}, 
	columns/P-AVG/.style ={column name=\approach{$_{\mathit{avgN}}$}}, 
	columns/P-FITI/.style={column name=\approach}, 
	columns/R-SC/.style ={column name=\approach{$_{\mathit{score}}$}}, 
	columns/R-TN/.style={column name=\approach{$_{\mathit{topN}}$}}, 
	columns/R-AVG/.style ={column name=\approach{$_{\mathit{avgN}}$}}, 
	columns/R-FITI/.style={column name=\approach}, 
	columns/F-SC/.style ={column name=\approach{$_{\mathit{score}}$}}, 
	columns/F-TN/.style={column name=\approach{$_{\mathit{topN}}$}}, 
	columns/F-AVG/.style ={column name=\approach{$_{\mathit{avgN}}$}}, 
	columns/F-FITI/.style={column name=\approach}, 
	col sep=comma,
	string type,
]{data/rq-selection.csv}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> pics/table-selection.tex <==
\pgfplotstabletypeset[
	every head row/.style={
		before row=\toprule,
		after row=\midrule,
	},
%	every nth row={4}{before row=\midrule},
	every last row/.style={
		after row=\bottomrule},
		columns/S/.style ={column name={ID}}, 
		columns/Group/.style ={column name={$s.\mathit{group}$}},
		columns/Avg/.style ={column name={$s.\mathit{avg}$}},
		columns/Max/.style ={column name={$s.\mathit{max}$}},
		columns/Word/.style ={column name={$s.\mathit{word}$}},
		columns/ML/.style ={column name={$s.\mathit{ml}$}},
		columns/Total/.style ={column name={$s.\mathit{score}$}
	}, 
	col sep=comma,
	string type,
]{data/selection.csv}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

